Efficient Adaptive Activation Rounding for Post-Training Quantization

Post-training quantization attracts increasing attention due to its convenience in deploying quantized neural networks. Although rounding-to-nearest remains the prevailing method for DNN quantization, prior research has demonstrated its suboptimal nature when applied to weight quantization. They propose optimizing weight rounding schemes by leveraging output error rather than the traditional weight quantization error. Our study reveals that similar rounding challenges also extend to activation quantization. Despite the easy generalization, the challenges lie in the dynamic nature of activation. Adaptive rounding is expected for varying activations and the method is subjected to runtime overhead. To tackle this, we propose the AQuant quantization framework with a novel perspective to reduce output error by adjusting rounding schemes of activations. Instead of using the constant rounding border 0.5 of the rounding-to-nearest operation, we make the border become a function w.r.t. the activation value to change the activation rounding by the adaptive border. To deal with the runtime overhead, we use a coarse-grained version of the border function. Finally, we introduce our framework to optimize the border function. Extensive experiments show that AQuant achieves notable improvements compared to state-of-the-art works and pushes the accuracy of ResNet-18 up to 60.31% under the 2-bit weight and activation quantization.

==> tex_files/Limitations.tex <==
\section{Limitations and Society Impacts}
\label{sec:limitations}

==> tex_files/archived.tex <==
\section{Try to use the theoretical framework of AdaRound to explain the activation rounding}
We now theoretically demonstrate that the rounding of activations should be dominated by the output MSE instead of themselves.
We follow the assumption (a) of AdaRound~\citep{nagel2020up} that activations among different layers are much less relevant than activations within each layer to simplify the analysis.
As such, we can analyze the perturbation of the activation in a layer-wise fashion. The effect of quantization error is formulated as 
\begin{equation}
\footnotesize
\begin{aligned}
&\mathop{\arg\min}\limits_{\Delta \mathbf{x}} \mathbb{E}[\mathcal{L}(\mathbf{x}+\Delta \mathbf{x}, \mathbf{y}, \mathbf{w})-\mathcal{L}(\mathbf{x}, \mathbf{y}, \mathbf{w})] \\
% {\approx} & \mathbb{E}\left[\Delta \mathbf{x}^{T} \nabla_{\mathbf{x}} \mathcal{L}(\mathbf{x}, \mathbf{y}, \mathbf{w}) +\frac{1}{2} \Delta \mathbf{x}^{T} \nabla_{\mathbf{x}}^{2} \mathcal{L}(\mathbf{x}, \mathbf{y}, \mathbf{w}) \Delta \mathbf{x}\right] \\
\stackrel{(a)}{\approx } & \mathop{\arg\min}\limits_{\Delta \mathbf{x}} \mathbb{E}\left[\Delta \mathbf{x}^{{(\ell)}^{T}} \mathbf{g}^{\left(\mathbf{x'}^{(\ell)}\right)} +\frac{1}{2} \Delta \mathbf{x}^{(\ell)^{T}} \mathbf{H}^{\left(\mathbf{x'}^{(\ell)}\right)} \Delta \mathbf{x}^{(\ell)}\right]\\
{\approx}& \mathop{\arg\min}\limits_{\Delta \mathbf{x}} \mathbb{E}\left[\frac{1}{2} \Delta \mathbf{x}^{(\ell)^{T}} \mathbf{H}^{\left(\mathbf{x'}^{(\ell)}\right)} \Delta \mathbf{x}^{(\ell)}\right],
\end{aligned}
\label{equ:adapt_to_activation}
\end{equation}
where $\mathbf{g}^{\left(\mathbf{x'}^{(\ell)}\right)}$ and $\mathbf{H}^{\left(\mathbf{x'}^{(\ell)}\right)}$ denote the first order derivative and Hessian matrix of the final loss $\mathcal{L}$ w.r.t. $\mathbf{x'}^{(\ell)}$. The first term is ignored because the gradient term approaches 0 when the model gets converged~\citep{nagel2020up}. Therefore, the second term defines the impact of the activation perturbation on the final loss $\mathcal{L}(\mathbf{x}, \mathbf{y}, \mathbf{w})$. Note that the inputs of layer $\ell$ contain errors caused by the quantization of previous layers, so that we use noised $\mathbf{x'}^{(\ell)}=\mathbf{x}^{(\ell)}+\mathbf{e}^{(\ell)}$ in Equation \ref{equ:complete_goal} instead of $\mathbf{x}$, and the $\Delta \mathbf{x}^{(\ell)}$ is the difference between $\mathbf{\hat{x'}}^{(\ell)}$ and $\mathbf{x}^{(\ell)}$. 
This \textbf{propagated error} is ignored by previous works~\citep{nagel2020up,li2020brecq,wei2022qdrop}, but it is important for adaptive activation rounding.
Equation \ref{equ:adapt_to_activation} cannot be directly optimized due to the computational complexity of the Hessian. We further expand the Hessian to find a way to approximate it. For two activations $x_a^{(\ell)}$ and $x_b^{(\ell)}$, the corresponding element in Hessian is
% \begin{equation}
% \begin{aligned}
% H_{x_{a}, x_{b}}^{(\ell)}=\frac{\partial^{2} \mathcal{L}}{\partial x_{a}^{(\ell)} \partial x_{b}^{(\ell)}} &=\frac{\partial}{\partial x_{b}^{(\ell)}}\left[\frac{\partial \mathcal{L}}{\partial \mathbf{z}^{(\ell)}} \frac{\partial \mathbf{z}^{(\ell)}}{\partial x_{a}^{(1)}}\right] \\
% &=\frac{\partial}{\partial x_{b}^{(\ell)}}\left[\left(\frac{\partial \mathcal{L}}{\partial \mathbf{z}^{(\ell)}}\right)^{T} \cdot \mathbf{W}_{:, a}^{(\ell)}\right] \\
% &=\mathbf{W}_{:, b}^{(\ell)^T} \frac{\partial^{2} \mathcal{L}}{\partial \mathbf{z}^{(\ell)^2}} \mathbf{W}_{:, a}^{(\ell)}.
% \end{aligned}
% \end{equation}
\begin{equation}
\footnotesize
\begin{aligned}
H_{x_{a}, x_{b}}^{(\ell)}=\frac{\partial^{2} \mathcal{L}}{\partial x_{a}^{(\ell)} \partial x_{b}^{(\ell)}} =\mathbf{W}_{:, b}^{(\ell)^T} \frac{\partial^{2} \mathcal{L}}{\partial \mathbf{x'}^{(\ell+1)^2}} \mathbf{W}_{:, a}^{(\ell)}.
\end{aligned}
\end{equation}
So that the Hessian matrix of activations $\mathbf{x'}^{(\ell)}$ is 
\begin{equation}
\footnotesize
\mathbf{H}^{\left(\mathbf{x'}^{(\ell)}\right)}=\mathbf{W}^{(\ell)^T} \frac{\partial^{2} \mathcal{L}}{\partial \mathbf{x'}^{(\ell+1)^2}} \mathbf{W}^{(\ell)}.
\end{equation}
The $\frac{\partial^{2} \mathcal{L}}{\partial \mathbf{x'}^{(\ell+1)^2}}$ requires backpropagation of second derivatives, which results in unbearable complexity. \citet{nagel2020up} shows that $\frac{\partial^{2} \mathcal{L}}{\partial \mathbf{x'}^{(\ell+1)^2}}$ is safe to be regarded as a diagonal constant matrix, denoted by $\operatorname{diag}\left(\nabla_{\mathbf{x'}^{(\ell+1)}}^{2} \mathcal{L}_{i, i}\right)$. We have
\begin{equation}
\footnotesize
\begin{aligned}
& \mathop{\arg\min}\limits_{\Delta \mathbf{x}} \mathbb{E}\left[\Delta \mathbf{x}^{(\ell)^{T}} \mathbf{H}^{\left(\mathbf{x'}^{(\ell)}\right)} \Delta \mathbf{x}^{(\ell)}\right]\\
\stackrel{(b)}{= } & \mathop{\arg\min}\limits_{\Delta \mathbf{x}} \mathbb{E}\left[\operatorname{diag}\left(\nabla_{\mathbf{x'}^{(\ell+1)}} \mathcal{L}_{i, i}\right)  \Delta \mathbf{x}^{(\ell)^{T}} \mathbf{W}_{i, :}^{(\ell)^{T}} \mathbf{W}_{i, :}^{(\ell)} \Delta \mathbf{x}^{(\ell)}\right] \\
= & \mathop{\arg\min}\limits_{\Delta \mathbf{x}} \mathbb{E}\left[\left(\mathbf{W}_{i, :}^{(\ell)} \Delta \mathbf{x}^{(\ell)}\right)^{2}\right].
\end{aligned}
\label{equ:activation_optimization_goal}
\end{equation}
Here, (b) requires $\Delta \mathbf{x}$ to be independently selected for different $\mathbf{W}_{i, :}^{(\ell)}$. The optimization of the final task loss decomposes into independent sub-problems in Equation \ref{equ:activation_optimization_goal}.  Each sub-problem deals with the VDP of $\mathbf{W}_{i, :}^{(\ell)}$ and $\mathbf{x'}^{(\ell)}$, resulting in the a single expected value of the output tensor.  This indicates that the quantization of activations is to minimize the output MSE of the next layer rather than the MSE themselves, which concludes our proof. 

~\citet{nagel2020up} has shown the quantization of weights should also minimize the output error. Then the optimization objective considering the quantization of both activations and weights is
\begin{equation}
\footnotesize
\begin{split}
& \mathop{\arg\min}\limits_{\Delta \mathbf{x'}, \Delta \mathbf{W}} \mathbb{E}\left[\left(\left(\mathbf{W}_{i, :}^{(\ell)}+\Delta \mathbf{W}_{i, :}^{(\ell)}\right)\left(\mathbf{x'}^{(\ell)}+\Delta \mathbf{x'}^{(\ell)}\right) \right. \right. \\
& \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \left. \left. -\mathbf{W}_{m ,:}^{(\ell)} \mathbf{x}^{(\ell)}\right)^{2}\right] \\
=& \mathop{\arg\min}\limits_{\Delta \mathbf{x'}, \Delta \mathbf{W}} \mathbb{E}\left[\left(\left(\mathbf{W}_{i, :}^{(\ell)}+\Delta \mathbf{W}_{i, :}^{(\ell)}\right) \Delta \mathbf{x'}^{(\ell)} +\Delta \mathbf{W}_{m ,:}^{(\ell)} \mathbf{x'}^{(\ell)} \right. \right.\\
& \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \left. \left. +\mathbf{W}_{i, :}^{(\ell)}\mathbf{e} \right)^{2}\right].
\label{equ:complete_goal}
\end{split}
\end{equation}
We eliminate full-precision $\mathbf{x}^{(\ell)}$ since they are unknown at runtime. Equation \ref{equ:complete_goal} quantitatively shows that the rounding of activations should be aware of the impact of weight quantization and the propagated errors. We assume $\Delta \mathbf{W}$ are given by the previous methods~\citep{nagel2020up,li2020brecq,wei2022qdrop} since they are out of the scope of this work.

% Based on Equation \ref{equ:complete_goal}, we aim to find an effective and light-weight way to round activations at the inference stage. 
 


